Garfield: System Support for Byzantine Machine Learning

We present Garfield, a library to transparently make machine learning (ML) applications, initially built with popular (but fragile) frameworks, e.g., TensorFlow and PyTorch, Byzantine-resilient. Garfield relies on a novel object-oriented design, reducing the coding effort, and addressing the vulnerability of the shared-graph architecture followed by classical ML frameworks. Garfield encompasses various communication patterns and supports computations on CPUs and GPUs, allowing addressing the general question of the very practical cost of Byzantine resilience in SGD-based ML applications. We report on the usage of Garfield on three main ML architectures: (a) a single server with multiple workers, (b) several servers and workers, and (c) peer-to-peer settings. Using Garfield, we highlight several interesting facts about the cost of Byzantine resilience. In particular, (a) Byzantine resilience, unlike crash resilience, induces an accuracy loss, (b) the throughput overhead comes more from communication than from robust aggregation, and (c) tolerating Byzantine servers costs more than tolerating Byzantine workers.

==> correctness.tex <==
\subsection{Correctness}
\label{subsec:proof}
The full formal specification of the \system{} protocol, along with its proof of correctness, is in~\cite{el2020genuinely}.
There, we formally show why our generic protocol works when instantiated with each GAR.  
Here we sketch intuitions of the correctness.

\begin{lemma}
\label{lemma:bounded_dev}
The expected maximum distance between parameter vectors on correct servers is always bounded.
\end{lemma}

\begin{proof}[Proof Sketch]
Based on our assumptions, the correct workers compute an unbiased estimate of the real gradient with a bounded variance, following a correct execution of the SGD algorithm.
Hence, the robust GAR (Step 7 in Figure~\ref{fig:asyncflowchart}) enables each parameter server to recover a \emph{correct} gradient (within an expected bounded range) from $n_w$ workers when a minority is Byzantine.
The key is that a robust GAR outputs a gradient which distance to any non-Byzantine gradient is bounded by a quantity \emph{independent} from the received Byzantine gradient.
For instance, when using \brute{} as a GAR, the following holds:
\begin{equation}
    \forall l \in H \mathsep
    \norm{\brute{}\left( x_{1} \ldotexp x_{n_w} \right) - x_l}
    \le \max\limits_{\left( i, j \right) \in {H}^2}{\norm{x_i - x_j}},
\end{equation}
where $x_k$ is the gradient estimated by worker $k$, and $l$,$i$, and $j$ are indices of \emph{correct} gradients belonging to the set $H$.
Hence, the distance between any two aggregated gradients (on two \emph{correct} servers) is bounded by the diameter of the correct gradients and so is the updated correct models (Step 8 in Figure~\ref{fig:asyncflowchart}), given that any correct server receives at least $f_w+1$ correct gradients (as $q_w \ge 2f_w+1$). 
Moreover, applying coordinate--wise \medianoid{}\footnote{Note that other Median--based aggregation techniques could be also used like \emph{mean around median} and \emph{trimmed mean}.} with $q_{ps} \geq 2f_{ps}+1$ ensures that the output model is bounded above and below by correct models, given at least $f_{ps}+1$ correct models are gathered.
This latter, fundamental piece for correctness is novel to the Byzantine SGD literature, which so far always relied on a single trusted server and only tolerated Byzantine fault at the workers' side.
\end{proof}

\begin{lemma}
\label{lemma:learning}
\system{} ensures the learning advancement towards a local minimum in each step.
\end{lemma}

\begin{proof}[Proof Sketch]
This relies on two fundamental pieces: (1) the computation of an unbiased gradient estimation on each correct worker and (2) the bounded deviation of parameter vectors on correct servers (Lemma~\ref{lemma:bounded_dev}). These two pieces result in the fact that the \emph{effective gradients} (which are used at the end to update the parameter vector sate) at the correct servers all lie in the same half-space as the true gradient. 
This ensures that all correct parameter vectors move towards a local minimum.
Applying coordinate--wise \medianoid{} (Step 10 in Figure~\ref{fig:asyncflowchart}) then outputs a vector in the range of correct vectors and hence, ensures that this output vector has advanced towards a local minimum.
In~\cite{el2020genuinely}, we formally prove the standard convergence criterion~\cite{bottou1998online}:
\begin{equation}
\label{eqn:final}
    \lim\limits_{t \rightarrow +\infty}{\expect\norm{\realgrad{\Bar{\params{}{t}}}}} = 0,
\end{equation}
where $\Bar{\params{}{t}}$ is the average of correct parameter vectors. 
\end{proof}

\begin{lemma}
Parameter vectors on correct servers are always confined beyond a bounded region.
\end{lemma}

\begin{proof}[Proof Sketch]
By the construction of the algorithm, all correct parameter servers start with the same random vector.
Based on Lemma~\ref{lemma:learning}, all vectors move in the same direction, which follows the same dynamics of vanilla SGD. Based on this, we can demonstrate that the second, third, and fourth moments of the \emph{effective gradients} are bounded with respect to the norm of the parameter vector on each correct worker, following the same standard proof of SGD~\cite{bottou1998online}. 
This essentially translates to the fact that the 
correct parameter vectors will remain confined within a bounded region. 
\end{proof}

\begin{lemma}
Eventually, all parameter vectors on correct servers contract almost--surely to the same values.
\end{lemma}

\begin{proof}[Proof Sketch]
Based on Lemma~\ref{lemma:learning}, all correct parameter vectors move towards a local minimum.
Given that the learning rate decreases with time, correct parameter vectors take smaller steps as they approach the local minimum.
Moreover, based on Lemma~\ref{lemma:bounded_dev}, we know that correct models are always close to each other.
As a result, after some time $t$, the expected maximum distance between correct vectors decreases over time, contracting eventually to the same vector (as a result of the repetitive application of \medianoid{} in each step).
Formally, \system{} ensures that the correct model parameters almost--surely converge to the same value:

\begin{equation}
\vspace{-2mm}
    \lim\limits_{t \rightarrow +\infty}{\expect\left( \max\limits_{\left( a, b \right) \in \range{1}{n_{ps} - f_{ps}}^2}\norm{\params{a}{t} - \params{b}{t}} \right)} = 0,
\end{equation}
where $\params{x}{t}$ is the parameter vector at server $x$ at time $t$.
\end{proof}

\begin{theorem}
\system{} achieves Byzantine--resilient learning with malicious servers and workers.
\end{theorem}
\begin{proof}[Proof Sketch]
Given all these previous lemmas, we can plug \system{} in the standard proof of SGD~\cite{bottou1998online}, showing convergence, despite the presence of Byzantine machines.
\end{proof}

==> garfield.tex <==

\section{The \system{} Framework}
\label{sec:async}

We first introduce the problem we tackle and our assumptions, then we describe the \emph{gradient aggregation rules} (GARs) implemented by \system{}.
Finally, we describe our protocol and discuss some intuitions about its Byzantine resilience. 

\input{prob_def}

\subsection{Assumptions}
We assume that the training data is distributed identically and independently \emph{(i.i.d)} on all workers~\cite{xing2015petuum}.
We assume $n_{ps} \ge 3f_{ps} + 1$, where the relation between $n_{w}$ and $f_{w}$ depends on the employed GAR (see Section~\ref{subsec:gars}).
We allow for a strong adversary that can coordinate Byzantine nodes and can delay communication or computation at correct nodes, but not indefinitely~\cite{castro1999practical}. In this sense, we do not assume any upper bound on the communication nor the computation time, i.e.,\ we assume an asynchronous network.

We assume the Byzantine nodes have strong, yet bounded, computation power and arbitrarily fast communication channels so as to compute the strong attacks presented in the ML literature~\cite{baruch2019little,bulyanPaper}. We also assume that these nodes have access to a subset of the training dataset and can overhear gradients sent by correct workers.
We assume that honest nodes can authenticate the source of a message to prevent spoofing and Sybil attacks. This can be done using public-key signatures~\cite{rivest1978method} and message authentication codes~\cite{tsudik1992message}. We assume that the adversary does not have enough computation power to break the cryptographic techniques~\cite{castro1999practical}.

\subsection{Statistically Robust GARs}
\label{subsec:gars}
In this section, we introduce the GARs implemented by \system{}. 
A GAR is merely a function of $\left( \setr^d \right)^q \rightarrow{} \setr^d$, with $d$ the dimension of the input vector (i.e.,\ a gradient or a model) space $\setr^d$ and $q$ the number of input vectors. 
Basically, these GARs wait for $q$ vectors before applying some functions on them.
Hence, in synchronous settings, these GARs can be deployed with $q$ machines in the system (so that the aggregator node can gather replies from \emph{all} nodes in the system within some time bound).
Yet, in asynchronous settings, one would require to deploy $q+f$ nodes to use these GARs, to ensure liveness of the protocol, where $f$ denotes the maximum number of Byzantine inputs.
In short, all GARs output a vector with special statistical properties that make them safe to use in the Byzantine setting.

\noindent{\textbf{1. \medianoid{}~\cite{xie2018generalized}}} computes the coordinate-wise median among the input gradients and outputs one gradient of these medians. 
\medianoid{} requires $q \ge 2f+1$, and its asymptotic complexity is $\mathcal{O}(qd)$.

\noindent{\textbf{2. \mkrum{}~\cite{aggregathor}}} assigns a \emph{score} (based on a sum of distances with the closest neighbors) to each gradient a worker submits to the server, and then returns the average of the smallest scoring gradients set of size $m$ (with $m\le q-f-2$). For aggregating workers' replies, \mkrum{}
achieves a better convergence rate compared to \medianoid{}~\cite{aggregathor}.
\mkrum{} requires $q \ge 2f+3$, and its asymptotic complexity is $\mathcal{O}(q^2d)$.

\noindent{\textbf{3. \brute{}~\cite{rousseeuw1985multivariate}}} finds a subset group of gradients of size $q - f$ with the minimum diameter among all other subsets, where the diameter of a group is defined as the maximum distance between any two gradients of this subset. \brute{} then outputs the average of the chosen subset.
Notably, \brute{} carries an exponential\footnote{Exponential when $f = \mathcal{O}\!\left( q \right)$, polynomial when $f = \mathcal{O}\!\left( 1 \right)$.} asymptotic complexity, in $\mathcal{O}\!\left( \binom{q}{f} + q^2 d \right)$.
Yet, as we will discuss later, its assumptions about variance are weaker than for the previous two GARs~\cite{mhamdi2019fast}.
\brute{} requires $q \ge 2f+1$.

\noindent{\textbf{4. \bulyan{}~\cite{bulyanPaper}}} robustly aggregates $q$ gradients by iterating several times (say $k$ times) over another Byzantine--resilient GAR, e.g.,\ \mkrum{}.
In each of these $k$ iterations, \bulyan{} extracts the gradients selected by such a GAR. 
Then, it computes the the coordinate-wise median of the $k$ selected gradients.
It then extracts the closest $k'$ gradients to the computed median, and finally returns the coordinate-wise average of these $k'$ gradients.
Unlike previous GARs, 
\bulyan{} can sustain a model with a large dimension.
Yet, it requires $q \ge 4f+3$, and its asymptotic complexity is $\mathcal{O}(q^2d)$.

\paragraph{Tradeoffs.}
In addition to the differences in the ratio of tolerated Byzantine nodes 
(inequalities relating $q$ with $f$)
and the computational cost of each GAR, the model dimension is also crucial in deciding which GAR to use.
For high dimensions (e.g.,\ order of millions), one should use \bulyan{}~\cite{bulyanPaper}.
In low dimensions, the application setup should satisfy the \emph{variance} assumption of the working GAR, as given below:
%\begin{equation*}
\begin{align*}
    \exists \kappa \in \left] 1, +\infty \right[ \mathsep \forall \left( i, t, \params{}{} \right) \in \range{1}{n-f} \times \setn \times \setr^d \mathsep \\
    \kappa \, \Delta \, \sqrt{\expect\left( \norm{\gradvar{i}{t} - \expect\gradvar{i}{t}}^2 \right)} \le \norm{\realgrad{\params{}{}}},
    \end{align*}
%\end{equation*}

where,
\begin{equation*}
    \Delta = \begin{cases}
        \frac{2 f}{n - f} &
        \text{if GAR = \brute{}} \\
        \sqrt{2 \left( n\!-\!f\!+\!\frac{f \left( n - f - 2 \right) + f^2 \left( n - f - 1 \right)}{n - 2 \, f - 2} \right)} &
        \text{if GAR = \mkrum{}} \\
        \sqrt{n-f} &
        \text{if GAR = \medianoid{},}
    \end{cases}
\end{equation*}
where $\gradvar{i}{t}$ is the estimated gradient by worker $i$ at time $t$, and $L(\theta)$ is the loss function at the model state $\theta$.
We provide a simple tool, \texttt{measure\_variance.py}, to estimate whether such a condition is satisfied.
Such a tool takes the experimental setup ($n$, $f$, the batch size, ..etc) as inputs. 
Then, it does few training steps, while estimating the true gradient $\realgrad{\params{}{}}$ by computing a gradient using a huge batch size.
In each training step, such a tool checks whether the condition stated above is satisfied or not, and then, gives the user statistics on how often such a condition is satisfied with each~GAR.

\input{protocol}

==> overview.tex <==
\lstset{language=Python}
\lstset{frame=lines}
\lstset{caption={Minimal example: it shows a simple example on using \system{}. These lines are copied from real working example. Some technical details are dropped for brevity.}}
\lstset{label={lst:min_ex}}
\lstset{basicstyle=\footnotesize}
\begin{lstlisting}
#1) Read command line parameters
ps_hosts = FLAGS.ps_hosts.split(",")
worker_hosts = FLAGS.worker_hosts.split(",")
num_ps = len(ps_hosts)
num_workers = len(worker_hosts)
max_steps = FLAGS.max_steps
task = FLAGS.task

#2) Instantiate the model
model = models.conv_cifar10(inputs=inputs,act_fn=
    activation_func, optimizer=builder_opt, epoch=True)
model.init()

#3) Start grpc server
service = TrainMessageExchangeServicer()
server = grpc.server(
    futures.ThreadPoolExecutor(max_workers=1000))
all_pb2_grpc.add_TrainMessageExchangeServicer_to_server(
    service, server)
server.add_insecure_port(ps_hosts[int(FLAGS.task_index)])
server.start()

#4) Initiate connections to all PSes and workers
for ps in ps_hosts:
	channel = grpc.insecure_channel(ps)
	stub = all_pb2_grpc.TrainMessageExchangeStub(channel)
	ps_conns.append(stub)

for worker in worker_hosts:
	channel = grpc.insecure_channel(worker)
	stub = all_pb2_grpc.TrainMessageExchangeStub(channel)
	worker_conns.append(stub)
	
if task='ps':
    # Instantiate the dataset
    dataset = datasets.load_cifar10()
    train_set = dataset.cut(0,50000, 50000).shuffle()
        .cut(0,50000, FLAGS.batch)
    test_set = dataset.cut(50000, 60000, 10000)

    # The training loop
    iter_num=0
    while iter_num < max_steps:
    	acc = model.eval(test_set)
    	create_complete_model()
    	grads = read_gradients()
    	grad = aggregate(grads)
    	model.update(grad)
    	iter_num+=1
else:
    # The training loop
    iter_num=0
    while iter_num < max_steps:
    	new_model = get_complete_model()
    	model.write(new_model)
    	grad = model.backprop()
    	iter_num+=1    
\end{lstlisting}


\section{\system{}: An Overview}
\label{sec:overview}
In this section, we describe a minimal training example that a programmer can write with the help of \system{} components which we describe in detail in Section~\ref{sec:arch}. Snippet~\ref{lst:min_ex} shows an example of a code that can be deployed and run on a set of machines (some run as parameter servers and other as workers) in a distributed environment. Below, we describe each part of this code snippet.

At the beginning of the experiment, the practitioner can extract the parameters of the experiment from the command line or equivalent. These parameters should include number of workers, number of parameter servers, the task type (whether a worker or a parameter server), and the number of learning steps. It can also include other hyper parameters like the learning rate, the used optimizer, dataset name, and model name. Based on the defined model and dataset, a user can initialize the experiment using the interface we provide.

Second, the user can define the networking abstractions required for her experiment. This includes initializing the gRPC service and starting the gRPC server\footnote{Not to confuse with parameter server. Both workers and parameter servers need to initialize this server to respond to requests from other machines.}. Next, the user should initiate connections with all other machines exist in the field, be workers of parameter servers.

In this example, the parameter server is assigned to manage the dataset and hence, it loads the dataset through the given interface and split this dataset into train and test sets. Practically, the dataset should not be managed by parameter servers only. Workers will never know if a Byzantine server is providing some malicious or poisoned data or not. But, for clarity purposes, the dataset is managed by the parameter servers.

On the one hand, the parameter server starts its training loop with preparing the latest model and the batch (from the dataset) that can be then pulled later by workers (different workers pull the same model but different batches of data). A server then waits for the workers to finish the gradient computation before reading these computed gradients. This process is abstracted in the function ``read\_gradients()". Afterwards, a server aggregates the received gradients to obtain one final gradient, using which it updates the model. This concludes one iteration on the parameter server side.

On the other hand, the training loop on the workers' side starts with reading the current model and the data batch from parameter server(s). Then, a worker saves the received model and compute gradients using the ``backprop" function. The resulting gradient is saved so that it can be sent back to the parameter server(s) when requested.

==> prob_def.tex <==
\subsection{Problem Definition}
\label{sec:prob_def}
Contrary to the standard parameter server scheme \cite{li2013parameter} where the server is a single point of failure, \system{} assumes $n_w$ workers and $n_{ps}$ servers, among which up to $f_w$ workers and $f_{ps}$ servers can behave arbitrarily.
The goal is for the correct nodes\footnote{When there is no ambiguity, we refer to both workers and parameter servers by \emph{nodes}.} to learn despite the $f_w + f_{ps}$ Byzantine nodes.
More concretely, \system{} devises a learning procedure (Figure \ref{fig:asyncflowchart}) that reaches a final parameter $\bm{x}_{opt}$ close to the one that would have been reached without Byzantine workers.
The problem is well-studied in Byzantine-free distributed systems, e.g.,\ \cite{colalearning} and systems with Byzantine workers, e.g.,\ \cite{lilisu2019, krum, alistarh2018byzantine, xie2018zeno}.
We list below the properties (using informal wording) that we identified to also tolerate Byzantine servers:
\begin{enumerate}
    \item \textbf{Bounded deviation.} Parameter vectors on correct servers should not deviate too much from each other.
    \item \textbf{Eventual contraction.} Parameter vectors on correct servers should eventually reach the same values.
    \item \textbf{Advancement of learning.} Before convergence (i.e.,\ before some step $t$), each correct parameter vector should come closer to the optimal solution after each step. In other words, the updating vector should have the same direction as the true gradient.
    \item \textbf{Global confinement.} Correct servers' parameter vectors should remain confined within a bounded region.
\end{enumerate}

The first and the last properties constitute the safety requirements; the rest are the liveness requirements.
All these requirements are both crucial and non-trivial to attain with the existing algorithms.
For instance, one would think of a solution in which each parameter server works on its own by collecting gradients from all workers and applying a statistically-robust GAR to filter out Byzantine replies.
Unfortunately, such a solution will not work as it will not ensure neither the \emph{bounded deviation} nor the \emph{eventual contraction} requirements and as a result, it is impossible to ensure advancement of learning in each step.
Intuitively, if parameter vectors on correct servers become arbitrarily far from each other, then the gradients of one vector (i.e.,\ model) cannot be used to update the state of another vector.
As a result, this novel setup requires a crucial novel requirement, which is the agreement among correct servers on the parameter vector at each step.
With the well--known impossibility result of agreement in Byzantine, asynchronous setup~\cite{fischer1985impossibility}, we rely on the abstraction of \emph{approximate agreement}~\cite{Fekete87} instead.

==> protocol.tex <==
\subsection{The \system{} Protocol}

Here we describe how \system{} works, highlighting how it tolerates Byzantine servers and workers while not assuming network synchrony. 

Figure~\ref{fig:asyncflowchart} displays a full training step and the communication involved.

\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth]{async-timeline}
\caption{One training loop in \system{}. The left line abstracts all parameter servers whilst the right line abstracts all workers. Arrows indicate communication. For instance, step 9 indicates exchanging the updated model among the server replicas.
The GAR at step 7 could be any of those presented in Section~\ref{subsec:gars}.
}
\label{fig:asyncflowchart}
\vspace{-4mm}
\end{figure}

\paragraph{Initialization.}

Each non--Byzantine parameter server initializes the model using the same \emph{seed} so that each of them can start with the same initial model.

\paragraph{Worker behavior.}

Each worker (1) gathers a \emph{subset} $q_{ps}$ of parameters from the first responding server replicas and (2) aggregates the received parameters using \medianoid{}.
Asynchrony, together with the presence of (at most) $f_{ps}$ Byzantine servers, makes it impossible for a worker to wait for more than $n_{ps} - f_{ps}$ parameter servers.
The intuition is that if it does, then the (possibly colluding) Byzantine servers would only need to never reply to stop the training.
Our protocol requires $2f_{ps} + 1 \le q_{ps} \le n_{ps} - f_{ps}$, 
and we consistently use $q_{ps} = 2f_{ps} + 3$ in our experiments.

\paragraph{Server behavior.}

Each server (1) gathers a \emph{subset} $q_w$ of gradients from the first responding workers and (2) robustly aggregates these gradients using any Byzantine--resilient GAR (Section~\ref{subsec:gars}) with $q_{w} \le n_{w} - f_{w}$ (due to asynchrony).
The server then uses the aggregated gradient to update the parameters (Equation \ref{eq:opt-step}). 
Servers then perform one more round of communication between each other (steps 9--11 in Figure \ref{fig:asyncflowchart}), in which they exchange their just--updated parameters.
Each server waits for $q_{ps} \ge 2f_{ps} + 1$ other parameter vectors and then aggregates them with its own using \medianoid{}. 
This additional step is paramount for correctness as
it bounds the expected maximal pairwise distance between any two parameters,
despite the impossibility of agreement in our asynchronous, Byzantine environment.

\input{correctness}

